Scaling Multi-Domain Dialogue State Tracking via Query Reformulation

We present a novel approach to dialogue state tracking and referring expression resolution tasks. Successful contextual understanding of multi-turn spoken dialogues requires resolving referring expressions across turns and tracking the entities relevant to the conversation across turns. Tracking conversational state is particularly challenging in a multi-domain scenario when there exist multiple spoken language understanding (SLU) sub-systems, and each SLU sub-system operates on its domain-specific meaning representation. While previous approaches have addressed the disparate schema issue by learning candidate transformations of the meaning representation, in this paper, we instead model the reference resolution as a dialogue context-aware user query reformulation task -- the dialog state is serialized to a sequence of natural language tokens representing the conversation. We develop our model for query reformulation using a pointer-generator network and a novel multi-task learning setup. In our experiments, we show a significant improvement in absolute F1 on an internal as well as a, soon to be released, public benchmark respectively.

==> discussion.tex <==
Although the above performance metrics are very promising, the LSTM system can suffer from overfitting in tail scenarios. I.e. the LSTM decoder may generatd completely irrelevant output that has no overlap with the input. In practice it may be possible to detect whether this happens by checking the percentage of words that were generated in the output by copying versus generation.

Another possible preprocessing that could improve the LSTM’s performance is to index the entities starting from the last contextual turn instead of the first.


There are two ways to understand why our auxilliary objective should work well.

A standard way to train the architecture that we described is to maximize the log0likelihood of some reference outputs given an input $x$. This method is also called teacher forcing. To mazimize the log0likelihood any of the stocahstic gradient based methods can be used after preforming back-propagation. But back-propagation will first pass through the decoder network and then through the encoder. This delays the rewards and can cause problems with learning.

The second way is that this enforces the encoder representation to directly be more infromative about the copy decision instead of relying on the decoder's language model for making that decision. 
One of the problems of this dataset, is that the exact words uttered by the user can be completely overwritten. Ideally what we want is that the rewrite should make minimal modifications to the utterance of the user.

